Neutron capture-induced silicon nuclear recoils for dark matter and CE$\nu$NS

Following neutron capture in a material there will be prompt nuclear recoils in addition to the gamma cascade. The nuclear recoils that are left behind in materials are generally below 1\,keV and therefore in the range of interest for dark matter experiments and CE$\nu$NS studies--both as backgrounds and calibration opportunities. Here we obtain the spectrum of prompt nuclear recoils following neutron capture for silicon.

==> authorinst.tex <==
\affiliation{School of Physics \& Astronomy, University of Minnesota, Minneapolis, Minnesota 55455, USA} 
\affiliation{Department of Physics, University of South Dakota, Vermillion, South Dakota 57069, USA} 

